Crowdsourced, Actionable and Verifiable Contextual Informational Norms

There is often a fundamental mismatch between programmable privacy frameworks, on the one hand, and the ever shifting privacy expectations of computer system users, on the other hand. Based on the theory of contextual integrity (CI), our paper addresses this problem by proposing a privacy framework that translates users' privacy expectations (norms) into a set of actionable privacy rules that are rooted in the language of CI. These norms are then encoded using Datalog logic specification to develop an information system that is able to verify whether information flows are appropriate and the privacy of users thus preserved. A particular benefit of our framework is that it can automatically adapt as users' privacy expectations evolve over time. To evaluate our proposed framework, we conducted an extensive survey involving more than 450 participants and 1400 questions to derive a set of privacy norms in the educational context. Based on the crowdsourced responses, we demonstrate that our framework can derive a compact Datalog encoding of the privacy norms which can in principle be directly used for enforcing privacy of information flows within this context. In addition, our framework can automatically detect logical inconsistencies between individual users' privacy expectations and the derived privacy logic.

==> ac.tex <==
%!TEX root = main.tex
\section{Access Control model}\label{sec:ac}

In the previous section we have outlines how our system uses Datalog to encode and evaluate norms. We now describe how it enforces norms onto posted information by using information-centric, space-based access control (AC) model.  

Since CI framework is described as a synchronous interaction between senders and receivers, previous efforts~\cite{barth2006privacy,criado2015implicit,krupa2012handling} have mimicked this by verifying each message against respective norms before its transmission. 

Conversely,  we opt for an asynchronous, space-based approach, motivated by the AC model in~\cite{shvartzshnaider2014moana}. In this model, policies (norms) are treated as views onto the information-space. This provide us with a coherent AC model that leaves the semantics (email, forum messages, tweets, posts)  to the applications themselves. 
%We leverage service and access control model suggested in~\cite{shvartzshnaider2014moana}, which is based on the following functional primitives: \verb+ADD+ and \verb+MAP+. The \verb+ADD+ functions adds 
In particular, in this model information is not explicitly sent  or transmitted to anyone in the traditional sense\footnote{By that we mean that information is not directly transferred from a specific  \emph{sender} to a \emph{recipient/s}}, rather it is added to  the global  information-space which can be then queried, e.g., users can run  a query that returns all information where they are stated as an intended  recipients. 

Using these primitives we define an AC model based on three conceptual views, namely: First view containing all the facts (i.e., information posts and norms). The second view results from running a query (i.e., applying norms) onto the first view, which will only contain information accessible by the requester. The third and final view is a result of a requester running a query on to the second view. The third view defines how informations lands onto the application logic. The third view is  outside the scope of this work.

This AC model maps naturally onto the ``Datalog world'', where information (facts) described as predicates, and implicitly added to the global information space. %along side the \emph{canView} predicates Listing~\ref{lbl:canView} which act as queries to retrieve all information complying with the norms. 

For readability, we slightly changed the CI semantics. Namely, we refer to the ``sender'' of the message as an \emph{Author} and the requester as the \emph{Viewer}. The rest of the attributes remain the same. %As a result, we use \emph{canView} predicate in Listing~\ref{lbl:canView} to query for information, which is complied with the norms.  %This significantly simplifies the development process because we don't need to go through
%\lstset{language=Prolog} 
%\begin{lstlisting}[caption={Example of a Post predicate}, style=myPrologstyle, label=lbl:post]  
%\begin{listing}
%\begin{minted}{prolog}
%post(classroom, 0, prateek, alice, 
%grade, none).
%
%agent(Agent) :- student(Agent).
%agent(Agent) :- professor(Agent).
%professor(Agent) :- 
%department_chair(Agent).
%
%professor(prateek).
%department_chair(sharad).
%student(alice).
%student(bob).
%\end{minted}
%\caption{Predicates.}
%\label{lbl:predicates}
%\end{listing}

%\lstset{language=Prolog} 
%\begin{lstlisting}[caption={Example of a Post predicate}, style=myPrologstyle, label=lbl:canView]
\begin{listing}
\begin{minted}[breaklines=true]{prolog}
canView(classroom, Viewer, PostID) :-
    % extract message data
    post(classroom, PostID, Author, Subject, Attribute, Transprin),
    % actual encoding of the norm
    allowed(classroom, Author, Viewer, Subject, grade, none).
\end{minted}
    \caption{canView predicate.}
    \label{lbl:canView}
\end{listing}
After defining a set of norms and encoding them into \emph{allowed} predicates, as described previously, we define a \emph{canView} predicate to query against the information space, as depicted by Listing~\ref{lbl:queries}. The \emph{canView} will return all posts that conform the \emph{allowed} clauses. 

\begin{listing}%[caption={Pretty-p}, style=myPrologstyle, label=lbl:query]
\begin{minted}{prolog}

%Alice can see in the classroom context:
?- canView(classroom, Alice, PostID), 
    post(classroom, PostID, Author, _, 
    	   grade, _).

\end{minted}
\label{lbl:queries}
\caption{Example of a queries}
\end{listing}

The last query in Listing~\ref{lbl:queries} is an example of essentially two queries:  the first view (global information space) is queried for information visible by Alice, next we query the resulting set  (i.e., the second view) for a particular information that is of interest to us (e.g., Post id, name of the Author, etc). 

The space-based, information-centric AC model is not defined by the applications running on top of it and can used to capture all of the existing information flows, as well as the new future ones. 

We now describe four distinct information flows founds in any information system: 

%====from the proposal

%(a) New messages; (b) Conditional
%information flows; (c) Transitive information flows; (d) Implicit
%information flows. We elaborate on each of these categories below.

\begin{figure}
\center
      \includegraphics[width= 0.5\textwidth]{direct.eps}
    \caption{Direct Information flow}
    \label{fig:direct}
\end{figure}



\begin{figure}
\center
      \includegraphics[width= 0.5\textwidth]{transitive.eps}
    \caption{Transitive Information flow}
    \label{fig:transitive}
\end{figure}

\begin{figure}
\center
      \includegraphics[width= 0.5\textwidth]{conditional.eps}
    \caption{Conditional Information flow}
    \label{fig:conditional}
\end{figure}

\begin{figure}
\center
      \includegraphics[width= 0.5\textwidth]{implicit.eps}
    \caption{Implicit Information flow}
    \label{fig:implicit}
\end{figure}
\begin{description} \setlength{\itemsep}{5pt}


\item[Direct flow] As depicted by Figure~\ref{fig:direct}, direct flow is established between two users. % A user who creates a post provides the requisitefields through the Compass interface.  
Every message at the time of creation is associated with a set of associated attributes including
the Author, the subject and the associated transmission principles. Unlike to a synchronous model where the message has to be verified fro privacy compliance for each receiver, in the asynchronous model, the recipients must first run a query to view the posts by the author, e.g,. by using Listing~\ref{lbl:queries}. The query will only return posts that the viewer is \emph{allow} to see. Any change in norms, is being reflected at the requesters' views. % For a create message, our system can directly use the
%Datalog privacy specification to test whether the information posting
%by the creator meets the context privacy specifications. Here, the
%subject corresponding to each message is explicitly specified in the
%message and the system first verifies whether the creator has the
%permissions to receive and post information corresponding to the
%subject, information type) pair. Every context has a defined set of transmission principles and the relevant set of transmissionprinciples can be determined given the (subject, information type) pair and the roles of the sender and recipient. 
%A new message sent to several recipients by a sender is individually verified for privacycompliance for each recipient.


\item[Conditional information flow] Transmission principles in context
privacy specifications can impose constraints for information
flow. 
%Not every message in Compass is immediately transmitted from the sender to a recipient; certain transmission principles have the power to restrict a transmission upon the condition of obtaining approval or a specific action from an actor in the system. 
For example, as depicted  by Figure~\ref{fig:conditional}, a professor may not have the privilege to transmit students' grades to
other actors without the consent of the student; such a transmission,
will be withheld by the system until the student provides explicit
consent from the respective student. While most conditional flows are
of the approval/consent type, certain transmission principles may
involve a set of actions by specific actors in the system and may
involve additional message transmissions. These additional message
transmissions which are triggered by transmission principles are
referred as {\em control messages} and are pre-defined in a given
context based on the transmission principle definitions.

The different semantic nature of these type of flows doesn't differ at the system level. This is just another an \emph{allowed} clause. In a case of an imposed condition, the  requester  will be able to  view the message only when the posed condition has been met and the result (i.e.,. approval/consent message, control messages) is posted back into the information-space.

\item[Transitive information flow] Reply or repost messages by users
in the system leads to indirect information flows beyond the original
creator of the information, shown in Figure \ref{fig:transitive}.  Whenever an indirect message traverses
new actors who are not in the original chain associated with the
creator leads to a transitive information flow.  

%
Similarly, at the system level, this flow is treated in a very similar manner to any other type flow. The replied or reposted messages are published  back to the information space, just as the original message, with slightly different attributes (i.e.,  different Author and Viewer). The semantics of the flows is left to the application layer. For example, a re-post, is a post with different author; threaded conversations is a query into the information space for all the messages that the \emph{Viewer} can see with a threaded interface implemented at the application layer by grouping the messaging  by different criteria, e.g., subject, date, etc.
%
%In Compass, every message is treated as an independent atomic unit associated with its own set of contextual integrity attributes. 

%Every reply or repost message automatically inherits all the contextual integrity attributes
%of the original message and the new additional attributes created by
%respondents. The system is designed in a way that a message and its
%response messages all belong the same information type and that the
%system does not conflate multiple information types. However, the
%subject corresponding to any repost becomes a list of actors including
%the original subject and potentially other subjects that have been
%added in the repost message. The sender list to any response or repost
%message is the entire chain of message transmitters including the
%creator of the thread. Every response and repost message is verified
%for (sender, recipient) pairs using the Datalog privacy specification
%for a given context for every (subject, information type) pair.  To
%enhance performance, Compass will cache the privacy computations of
%previous transmissions in a given thread of message responses to
%restrict the verification overhead. 

\item[Implicit information flow]
Certain message flows in the system
are implicit where the sender does not explicitly ``transmit" the message
to the recipient. Implicit information flows are of two kinds: (a)
system pre-configured; (b) pull-based. One example of a system
pre-configured implicit flow is one where some users may configure
their settings to allow other users to view their current status
information including location. A pull-based information flow is one where another user explicitly requests information about messages posted by another user.  A common example of such a flow is {\em search} of posts by a user.  As depicted by Figure~\ref{fig:implicit}, in  a space-based model, every new message exists  as part of a global information space, thus it intrinsically supports both types of such an information flow.


%While pull-based information flow can be supported
%in the same manner a normal information flow, the operation can be
%inefficient if the system has to verify the privacy constraints across
%all messages in the system.  To support implicit information flow
%efficiently, the Datalog information flow verification engine can
%compute a {\em digest} for every message posted in the system which is
%a pre-computed list of actors in a given context that can access a
%specific message. Upon the completion of specific conditional actions
%that relate to a message, the digest list can be updated. Precomputing
%the digest can significantly reduce search time, since the search
%operation is simplified to identifying message postings that match a
%search query and then filtering these messages based on their privacy
%digests that limit message visibility. Posts that require conditional 
%access are not displayed as search results.

%==============

\end{description}


==> datalog.tex <==
%!TEX root = main.tex
\section{Model} \note[Yan]{Brainstorming...looking at ways to model norms so we can reason with it}

Norm space is a framework which is built on header space analysis presented in~\cite{}. Similarly to header space framework where each norm is represented as a point in a geographical space.

We now define the head space $\{0,1\}^L$, where L represents a maximum length of the norm. We cross product the norms and the possible outcomes $\{0,1\}^L \times \{1...O\}$ where
$\{1...O\}$ represents a space set of  possible outcomes such as yes (1), no (0), don't know (3). Transfer function, $T$, transfers \emph{norm}, n, to specific outcome, o.
A collection of norms form a privacy policy, $P$ which is modeled as $T(n,o) : (n,o) \rightarrow \{(n_1, o_1), (n_2, o_2), ...\}$. The overall policies can be modeled as:

\begin{equation*}
\rho(n,o) = 
\begin{cases}
 P_1 (n, o) &  if o \in Context_1\\
 ...  &   ...\\
 P_2 (n, o)  & if o \in Context_n
 \end{cases}
\end{equation*}

Context transfer function???

==> logic_generation.tex <==
%!TEX root = main.tex
\section{Model} \note[Yan]{Brainstorming...looking at ways to model norms so we can reason with it}

Norm space is a framework which is built on header space analysis presented in~\cite{}. Similarly to header space framework where each norm is represented as a point in a geographical space.

We now define the head space $\{0,1\}^L$, where L represents a maximum length of the norm. We cross product the norms and the possible outcomes $\{0,1\}^L \times \{1...O\}$ where
$\{1...O\}$ represents a space set of  possible outcomes such as yes (1), no (0), don't know (3). Transfer function, $T$, transfers \emph{norm}, n, to specific outcome, o.
A collection of norms form a privacy policy, $P$ which is modeled as $T(n,o) : (n,o) \rightarrow \{(n_1, o_1), (n_2, o_2), ...\}$. The overall policies can be modeled as:

\begin{equation*}
\rho(n,o) = 
\begin{cases}
 P_1 (n, o) &  if o \in Context_1\\
 ...  &   ...\\
 P_2 (n, o)  & if o \in Context_n
 \end{cases}
\end{equation*}

Context transfer function???
